Do LLMs Build Spatial World Models? Evidence from Grid-World Maze Tasks

Foundation models have shown remarkable performance across diverse tasks, yet their ability to construct internal spatial world models for reasoning and planning remains unclear. We systematically evaluate the spatial understanding of large language models through maze tasks, a controlled testing context requiring multi-step planning and spatial abstraction. Across comprehensive experiments with Gemini-2.5-Flash, GPT-5-mini, Claude-Haiku-4.5, and DeepSeek-Chat, we uncover significant discrepancies in spatial reasoning that challenge assumptions about LLM planning capabilities. Using chain-of-thought prompting, Gemini achieves 80-86% accuracy on smaller mazes (5x5 to 7x7 grids) with tokenized adjacency representations, but performance collapses to 16-34% with visual grid formats, which is a 2-5x difference, suggesting representation-dependent rather than format-invariant spatial reasoning. We further probe spatial understanding through sequential proximity questions and compositional distance comparisons. Despite achieving 96-99% semantic coverage in reasoning traces, models fail to leverage this understanding for consistent spatial computations, indicating that they treat each question independently rather than building cumulative spatial knowledge. Our findings based on the maze-solving tasks suggest that LLMs do not develop robust spatial world models, but rather exhibit representation-specific and prompting-dependent reasoning that succeeds only under narrow conditions. These results have critical implications for deploying foundation models in applications requiring spatial abstraction.

==> conclusion.tex <==
In extending representational alignment inquiry to spatial world models, we provide empirical evidence that current LLMs lack representation-aligned spatial abstractions. Despite operating over identical underlying maze topologies, models exhibit dramatic performance collapses when the input representation shifts from adjacency lists to visual grid formats. This sensitivity suggests that success on spatial planning tasks arises from representation-specific heuristics rather than from an aligned internal spatial model capable of supporting format-invariant reasoning. Moreover, the observed failure to reuse spatial knowledge across sequential queries further indicates a lack of persistent, aligned representations—consistent with prior findings in ToM and relational reasoning domains.

Our proposed evaluation framework explicitly disentangles spatial reasoning from spatial planning, and systematically varies representation format, prompting strategy, and task composition. By combining maze navigation with sequential proximity queries and compositional distance comparisons, we directly test whether models build persistent, format-invariant spatial world models. The consistent failure of models to generalize across representations or reuse spatial knowledge positions our benchmark as a diagnostic tool for identifying representation-dependent reasoning—a critical limitation of current foundation models.
